Device Heterogeneity in Federated Learning: A Superquantile Approach

We propose a federated learning framework to handle heterogeneous client devices which do not conform to the population data distribution. The approach hinges upon a parameterized superquantile-based objective, where the parameter ranges over levels of conformity. We present an optimization algorithm and establish its convergence to a stationary point. We show how to practically implement it using secure aggregation by interleaving iterations of the usual federated averaging method with device filtering. We conclude with numerical experiments on neural networks as well as linear models on tasks from computer vision and natural language processing.

==> fig/main_schematic.tex <==

\begin{tikzpicture}[scale=0.15,
servernode/.style={ellipse, draw=black, fill=Goldenrod!10, very thick, minimum size=7mm},
devicenode/.style={rectangle, draw=black!60, very thick, minimum size=5mm, aspect=1.62},
secaggnode/.style={circle, draw=black, very thick, minimum size=1mm, fill=Lavender!10},
]

\tikzset{mark size=8pt} % size of plot mark
\tikzstyle{linesty1} = [cyan, very thick]
\tikzstyle{linesty2} = [BurntOrange, ultra thick, densely dotted]
\tikzstyle{linesty3} = [ForestGreen, ultra thick, dashdotted]
\tikzstyle{linesty4} = [OrangeRed, ultra thick, dashed]
\tikzstyle{linesty1s} = [cyan!75, very thick]
\tikzstyle{linesty2s} = [BurntOrange!75, ultra thick, densely dotted]
\tikzstyle{linesty3s} = [ForestGreen!75, ultra thick, dashdotted]
\tikzstyle{linesty4s} = [OrangeRed!75, ultra thick, dashed]
\tikzstyle{rectsty0} = [fill=gray!15, very thick]
\tikzstyle{rectsty1} = [fill=cyan!10, very thick]
\tikzstyle{rectsty2} = [fill=BurntOrange!10, very thick]
\tikzstyle{rectsty3} = [fill=ForestGreen!10, very thick]
\tikzstyle{rectsty4} = [fill=OrangeRed!10, very thick]

% \draw[thin, -] (-1, -1) rectangle (101, 51); % figure boundary

\node at (25,48) {\textbf{Trajectories of 
model parameters over time}};  % point is center of text


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\draw[thick, -] (5, 10) -- (45, 10); % x-axis
\draw[thick, -] (5, 10) -- (5, 33); % y-axis
\node at (24,7) {Iteration $\to$}; % x-label
\node[rotate=90] at (3, 22) {Model parameters $\to$}; %y-label

% legend
\draw[thin, -] (5, 1) rectangle (45, 5);
\draw[linesty1] (6,3) -- (10, 3);
\node  at (11.5,3) {$\theta_1$};

\draw[linesty2] (16,3) -- (20, 3);
\node  at (21.5,3) {$\theta_2$}; 

\draw[linesty3] (26,3) -- (30, 3);
\node  at (31.5,3) {$\theta_3$}; 

\draw[linesty4] (36,3) -- (40, 3);
\node  at (41.5,3) {$\theta_4$}; 

% curve #1
\draw [linesty1] plot [smooth] coordinates {(10.0, 27.0) (18.0, 31.5) (30.0, 25.5) (33.5, 26.2) (35.0, 25.7) (36.0, 26.2) (37.0, 25.7) (38.0, 26.2) (39.0, 25.7) (40.0, 26.0) };
\draw [linesty1] plot [only marks, mark=*] coordinates {(40,26)};
\node[outer sep=2pt] at (42.5,26) {$w_{\scriptscriptstyle\theta_1}$};

% curve #2
\draw [linesty2] plot [smooth] coordinates {(10.0, 27.0) (16.0, 29.0) (28.0, 20.0) (33, 22.5) (35.0, 21.8) (36.0, 21.9) (37.0, 22.1) (38.0, 21.8) (39.0, 22.1) (40.0, 22.0) };

\draw [linesty2] plot [only marks, mark=square*] coordinates {(40,22)};
\node[outer sep=2pt] at (42.5,22) {$w_{\scriptscriptstyle\theta_2}$};

% curve #3
\draw [linesty3] plot [smooth] coordinates {(10.0, 27.0) (15.0, 26.0) (26.0, 15.0) (33.0, 18.0) (34.4, 18.5) (36.0, 17.8) (37.0, 18.1) (38.0, 17.9) (39.0, 18.2) (40.0, 18.0) };

\draw [linesty3] plot [only marks, mark=diamond*] coordinates {(40,18)};
\node[outer sep=2pt] at (42.5,18) {$w_{\scriptscriptstyle\theta_3}$};


% curve #4
\draw [linesty4] plot [smooth] coordinates {(10.0, 27.0) (15.0, 27.0) (27.0, 12.0) (32.0, 13.5) (33.0, 14.0) (35.0, 13.7) (36.0, 14.2) (37.0, 13.8) (38.0, 14.1) (39.0, 13.9) (40.0, 14.05) };

\draw [linesty4] plot [only marks, mark=pentagon*] coordinates {(40,14)};
\node[outer sep=2pt] at (42.5,14) {$w_{\scriptscriptstyle\theta_4}$};

% w_0
\fill (10,27) circle[radius=0.5];
\node[outer sep=2pt] at (8,27) {$w_0$};


% Highlighting rectangle
\draw  [fill=RoyalPurple!50,draw=gray!50, opacity=0.25]  (25, 10) rectangle (27, 33) ;
\node[outer sep=2pt] at (26,9) {${t}$};
\node[draw=black!0] (highlight_rect) (26, 33) {}; % dummy node for location


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Training time
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node (trainlabel) at (75,48) {\textbf{In iteration $t$ of training}};  % point is center of text
% \fill (75,40) circle[radius=0.5];


% Server
\node[servernode] (trainserver) [below=1pt of trainlabel] {Server};

\node[secaggnode,scale=0.8] (sec_agg) [below=15pt of trainserver] {$\bm{+}$};

\node  at ([xshift=150pt,yshift=-10pt]sec_agg.north) {\scriptsize{Sec.Agg.}}; 

%nodes
\node[devicenode, rectsty0] (traindev2) [below=20pt of sec_agg] {};
\node[devicenode, rectsty0] (traindev1) [left=of traindev2] {};
\node[devicenode, rectsty0] (traindev3) [right=of traindev2] {};

\node  [left=0.1pt of traindev1, yshift=3.5pt] {\scriptsize{selected}};
\node  [left=0.1pt of traindev1, yshift=-3.5pt] {\scriptsize{devices}};


% node1
\draw[->,linesty4s] ([xshift=30pt]traindev1.north) to [bend left=10] ([xshift=10pt,yshift=-30pt]sec_agg.west) ;

\draw[->,linesty3s] ([xshift=10pt]traindev1.north) to [bend left=20] ([xshift=5pt,yshift=-10pt]sec_agg.west) ;

\draw[->,linesty2s] ([xshift=-10pt]traindev1.north) to [bend left=30] ([xshift=0pt,yshift=5pt]sec_agg.west) ;

\draw[->,linesty1s] ([xshift=-30pt]traindev1.north) to [bend left=40] ([xshift=3pt,yshift=20pt]sec_agg.west) ;


% node2
\draw[->,linesty4s] ([xshift=30pt]traindev2.north) to [bend right=20] ([xshift=22.5pt,yshift=0pt]sec_agg.south) ;

\draw[->,linesty3s] ([xshift=10pt]traindev2.north) to [bend right=10] ([xshift=7.5pt,yshift=0pt]sec_agg.south) ;

\draw[->,linesty2s] ([xshift=-10pt]traindev2.north) to [bend left=10] ([xshift=-7.5pt,yshift=0pt]sec_agg.south) ;

\draw[->,linesty1s] ([xshift=-30pt]traindev2.north) to [bend left=20] ([xshift=-22.5pt,yshift=0pt]sec_agg.south) ;

% node3
\draw[->,linesty4s] ([xshift=30pt]traindev3.north) to [bend right=40] ([xshift=-3pt,yshift=20pt]sec_agg.east) ;

\draw[->,linesty3s] ([xshift=10pt]traindev3.north) to [bend right=30] ([xshift=0pt,yshift=5pt]sec_agg.east) ;

\draw[->,linesty2s] ([xshift=-10pt]traindev3.north) to [bend right=20] ([xshift=-5pt,yshift=-10pt]sec_agg.east) ;

\draw[->,linesty1s] ([xshift=-30pt]traindev3.north) to [bend right=10] ([xshift=-10pt,yshift=-30pt]sec_agg.east) ;

% to server
\draw[->,linesty4s] ([xshift=30pt]sec_agg.north) to [bend right=20] ([xshift=22.5pt,yshift=0pt]trainserver.south) ;

\draw[->,linesty3s] ([xshift=10pt]sec_agg.north) to [bend right=10] ([xshift=7.5pt,yshift=0pt]trainserver.south) ;

\draw[->,linesty2s] ([xshift=-10pt]sec_agg.north) to [bend left=10] ([xshift=-7.5pt,yshift=0pt]trainserver.south) ;

\draw[->,linesty1s] ([xshift=-30pt]sec_agg.north) to [bend left=20] ([xshift=-22.5pt,yshift=0pt]trainserver.south) ;

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Test time
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node (testlabel) at (75,20) {\textbf{At test time}};  % point is center of text
% \fill (75,40) circle[radius=0.5];



% Server
\node[servernode] (testserver) [below=1pt of testlabel] {Server};

%nodes
\node[devicenode,rectsty2] (testdev3) [below=of testserver] {};
\node[devicenode,rectsty3] (testdev2) [left=of testdev3] {};
\node[devicenode,rectsty1] (testdev1) [left=of testdev2] {};
\node[devicenode,rectsty1] (testdev4) [right=of testdev3] {};
\node[devicenode,rectsty4] (testdev5) [right=of testdev4] {};

\draw[->,linesty1] (testserver.south) -- ([yshift=10pt,xshift=5pt]testdev1.north);
\draw[->,linesty3] (testserver.south) -- ([yshift=5pt]testdev2.north);
\draw[->,linesty2] (testserver.south) -- (testdev3.north);
\draw[->,linesty1] (testserver.south) -- ([yshift=5pt]testdev4.north);
\draw[->,linesty4] (testserver.south) -- ([xshift=-5pt,yshift=10pt]testdev5.north);

\node  [below=-4pt of testdev3, label={[align=center]below:\scriptsize{test devices select their level of conformity $\theta$}}] {};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arrow
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[-latex,thin, dashed] (26, 33.2) to [bend left=10] (trainlabel.west);



\end{tikzpicture}
